Wav2SQL: Direct Generalizable Speech-To-SQL Parsing

Speech-to-SQL (S2SQL) aims to convert spoken questions into SQL queries given relational databases, which has been traditionally implemented in a cascaded manner while facing the following challenges: 1) model training is faced with the major issue of data scarcity, where limited parallel data is available; and 2) the systems should be robust enough to handle diverse out-of-domain speech samples that differ from the source data. In this work, we propose the first direct speech-to-SQL parsing model Wav2SQL which avoids error compounding across cascaded systems. Specifically, 1) to accelerate speech-driven SQL parsing research in the community, we release a large-scale and multi-speaker dataset MASpider; 2) leveraging the recent progress in the large-scale pre-training, we show that it alleviates the data scarcity issue and allow for direct speech-to-SQL parsing; and 3) we include the speech re-programming and gradient reversal classifier techniques to reduce acoustic variance and learned style-agnostic representation, improving generalization to unseen out-of-domain custom data. Experimental results demonstrate that Wav2SQL avoids error compounding and achieves state-of-the-art results by up to 2.5\% accuracy improvement over the baseline.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% add in ICLR 2022
\def\eps{{\epsilon}}
\newcommand{\beps}{\boldsymbol\epsilon}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\bzeta}{\boldsymbol\hat{\beta}}
\newcommand{\talpha}{\tilde{\alpha}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\hat{\beta}}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/abstract/main.tex <==
\begin{abstract}
    Speech-to-SQL (S2SQL) aims to convert spoken questions into SQL queries given relational databases, which has been traditionally implemented in a cascaded manner while facing the following challenges: 1) model training is faced with the major issue of data scarcity, where limited parallel data is available; and 2) the systems should be robust enough to handle diverse out-of-domain speech samples that differ from the source data. In this work, we propose the first direct speech-to-SQL parsing model Wav2SQL which avoids error compounding across cascaded systems. Specifically, 1) to accelerate speech-driven SQL parsing research in the community, we release a large-scale and multi-speaker dataset MASpider; 2) leveraging the recent progress in the large-scale pre-training, we show that it alleviates the data scarcity issue and allow for direct speech-to-SQL parsing; and 3) we include the speech re-programming and gradient reversal classifier techniques to reduce acoustic variance and learned style-agnostic representation, improving generalization to unseen out-of-domain custom data. Experimental results demonstrate that Wav2SQL avoids error compounding and achieves state-of-the-art results by up to 2.5\% accuracy improvement over the baseline.
\end{abstract}

==> sections/conclusion/main.tex <==
\section{Conclusion}
We released MASpider, the first large-scale, multi-speaker, and multi-accent S2SQL parsing dataset, which we hope would accelerate S2SQL research in the community. In this work, we presented the first direct speech-to-SQL model Wav2SQL which avoided error compounding across cascaded systems. To tackle the data scarcity issue, we leveraged recent progress in large-scale pre-training and utilized self-supervised models to derive discriminate representation. To promote model generalization and robustness to custom out-of-distribution data, we further introduced speech re-programming and gradient-reversal classifier techniques which reduced acoustic variance and learned style-agnostic representations. Experimental results demonstrated that our approach achieved new state-of-the-art results by up to 4.6\% accuracy improvement over baseline. In the future, we will investigate techniques to further enhance the model generalization in direct Speech-to-SQL parsing.

==> sections/dataset/collection.tex <==
\subsection{Data Collection and Verification}


\textbf{Collection Procedure}
For all 9693 utterance-SQL pairs in MASpider, we ensure that each speaker is assigned no more than 1500 sentences to avoid excessive data distribution bias. Next, we collect the audio sample of the given text utterances in a professional recording studio. Finally, the spoken utterances are saved in wav format, sampled at 16kHz, and quantized by 16 bits. 


\textbf{Data Labeling}
For further study, we tag additional statistics such as the native language and age of the speakers, and the year of their English study. Following this, the dataset is split into 12-hour spoken questions for training, additional 3-hour utterances with unseen accents, speakers, and databases for testing, which enable the evaluation of model generalization to custom data. Figure~\ref{fig:split} illustrates the distribution of the training and test sets on MASpider.


\textbf{Data Verification}
Firstly, we check that the accent in the recording matches the speaker's country. Then, We listen to every recording to check for mispronounced errors and re-record the recording with more than two mispronunciations. Finally, we run the preliminary qualified recordings through an ASR system to control the recorded audio quality. In our case, we used the fine-tuned wav2vec 2.0 ASR model to filter out recordings with their character error rates higher than 25$\%$. For audio with these error rates above the threshold, it is discarded and recollected again until passed.


==> sections/dataset/main.tex <==
\section{Dataset Construction}
We build MASpider upon the Spider~\cite{yu2018spider}, which has 8659/1034 train/evaluation splits and an unreleased test set.
MASpider consists of 9693 spoken utterances recorded by eleven speakers from six different countries. MASpider consists of 15 hours of speech samples recorded in a professional recording studio, including 8.1 hours from 6 females and 6.9 hours from 5 males apart from the person-of-interest (POI). Figures~\ref{fig:stat} summarize the distribution of dataset split, gender, and country. More details on MASpider are available in the appendix~\ref{app:dataset}. The major features of MASpider include:

\begin{itemize}
    \item Open source. A lack of data could hinder the construction of speech-to-SQL systems, so we release our corpus to accelerate research in the community.
    \item Diversity. Since the distribution of custom voice could be different from training data, we construct a dataset with different gender, accent and language background to improve model generalization.
    \item High quality. High-quality audios without 
    excessive noise or error annotation are essential for S2SQL training. A strict verification ensures high-quality utterances in MASpider.
\end{itemize}
\input{sections/dataset/collection}
\begin{figure*}[htbp]
    \centering
    % \small
    \vspace{-8mm}
    \includegraphics[width=0.6\textwidth,trim={1.0cm 0cm 1.0cm 0cm}]{figs/model.png}
    \vspace{-3mm}
    \caption{The information flow with dotted lines is included during training. Subfigure(a) denotes the implementation process of Speech Re-programming $RR$: random resamling; $RPS$: a chain function for random pitch shifting of raw waveform. Subfigure(b) is the overall architecture of our Wav2SQL $RAT$: relation-aware transformer.}
    \label{fig:2}
\end{figure*}
\input{sections/dataset/statistics}

We build MASpider upon the Spider whose train/evaluation division is 8569/1034 and testset is not released. For this reason, MASpider consists of 9693 spoken utterances recorded by 11 speakers from six different countries. MASpider consists of 15 hours of speech samples recorded in a professional recording studio, including 8.1 hours from 6 females and 6.9 hours from 5 males apart from the person-of-interest (POI). Figures summarize the distribution of dataset split, gender, and country. More details about MASpider can be found in the appendix.



==> sections/dataset/statistics.tex <==
\subsection{Dataset Statistics}
After the data collection and processing procedure, we check for audio quality and conduct the statistical evaluation.

\textbf{Gender} The visualization of gender statistics is displayed as Figure~\ref{fig:gender}. As we can see, the ratio of male to female speakers is relatively average.

\textbf{Country} The recorders mainly include 4 English native speakers and 7 non-native speakers from Japan, China, Thailand, and Korea. We count the proportion of utterances recorded by these speakers and visualize it as shown in Figure~\ref{fig:country}


\textbf{Group By Difficulty}  Following the common practice~\cite{yu2018spider} to better demonstrate the model performance on different SQL queries, we group the difficulty of each spoken question into 4 levels according to the number of SQL components, selections, and conditions. Specifically, SQL queries that contain more keywords (e.g., GROUP BY, ORDER BY, INTERSECT, etc.) will be considered harder. In the end, The test set of MASpider consists of 25.5$\%$ easy, 37.9$\%$ medium, 20.9$\%$ hard, and 15.7$\%$ extra hard SQL queries. 

==> sections/experiment/ablation.tex <==
\subsection{Ablation Studies}
As shown in Table~\ref{res:1}, we conduct ablation studies to demonstrate the effectiveness of several designs in our model, including speech re-programming and gradient reversal classifier technique, and text schema linking. The results have been presented in Table \ref{res:1}, and we have the following discovering: 1) the speech re-programming methods show an improvement in exact match accuracy by 1.9\% and a substantial increase of 8.7\% in ORDER BY component matching, indicating its efficiency in reducing acoustic variance and learning deterministic representations; 2) Removing the gradient reversal classifier has witnessed a distinct degradation in model performance by 1.1\% accuracy especially in ORDER By component matching (1.6\%), showing its superiority in learning speaker-agnostic speech representation; 
% 3) Replacing rough ASR schema linking with text schema linking has witnessed the performance increase by up to 14.3 points in exact match accuracy, demonstrating that the schema linking is quite important in Speech-to-SQL parsing task.
% 3) Removing cross-modality fusion between the question (audio modal) and schema (text modal) has witnessed the performance decrease by up to 3 points in SELECT component matching and 2 points in exact match accuracy, demonstrating that the audio and textual modality gap could be reduced with the cross-modality fusion.

==> sections/experiment/case.tex <==
\subsection{Case Study}

We compare the SQL query generated by Wav2SQL with the baseline cascaded system in Table~\ref{table:case}. As shown in the table, we can notice that Wav2SQL has better performance than the baseline system, mainly in SELECT, WHERE, and KEYWORDS operations. For example, in the first and third cases, the cascading system fails to fill the values into the correct slots, thus, it stupidly forgets the 'Name' of table 'Singer' and is unable to select the correct column name(i.e, "Age"). In addition, Wav2SQL successfully completes the averaging operation on "Age" in the third case. Unfortunately, in the second example, the cascaded system incorrectly constructs the WHERE clause so that it fails to pick singers who are older than the average age.

==> sections/experiment/custom.tex <==
\subsection{Generalization To Custom Data}
For out-of-domain testing, we prepare spoken questions with databases, accents, and speakers that are unseen in custom data. The results are summarized in Table~\ref{res:1}, and we have the following observations:  1) As shown in the table, we see that our proposed Wav2SQL outperforms DeepSpeechSQL by a large margin of 16.4\% on exact match accuracy. In addition, the component matching of our model on all SQL components outperforms DeepSpeechSQL, especially in SELECT, GROUP BY, and ORDER BY components by 20.1\%, 26.0\%, and 44.2\%; 2) 
Under the challenge of invisible accents, Wav2SQL can still maintain competitive results with a 1.8\% exact match accuracy drop compared with the cascaded system, which validates the superiority of our model by exploiting speech re-program and adversarial training to get deterministic representations invariant to accents and speakers; 3) Although we are pleasantly surprised to find that we have a small gap with S2SQL-TTS in ELECT, GROUP BY and AND/OR component matching, there is still a certain gap with it in exact match accuracy, and we will further narrow this gap in future work. 

==> sections/experiment/main.tex <==
\section {Experiments}
% \vspace{-3mm}
\input{sections/experiment/setup}
\begin{table*}[h]
    \centering
    \small
    \begin{tabular}{l}
    \toprule
    \textbf{Medium}: Show name, country, age for all singers ordered by age from the oldest to the youngest. \\
    \textbf{Cascaded}: SELECT \textcolor{red}{singer.Country, singer.Age} FROM singer ORDER BY singer.Age Desc \\
    \textbf{Wav2SQL}: SELECT \textcolor{blue}{singer.Name, singer.Country, singer.Age} FROM singer ORDER BY singer.Age Desc \\
    \textbf{Gold SQL}: SELECT Name, Country, Age FROM singer ORDER BY Age Desc \\
    \midrule
    \textbf{Hard}: List all song names by singers above the average age.\\
    \textbf{Cascaded}: SELECT singer.Song\_Name FROM singer WHERE singer.Age < \textcolor{red}{'terminal' ORDER BY singer.Song\_Name Asc} \\
    \textbf{Wav2SQL}: SELECT singer.Song\_Name FROM singer WHERE singer.Age > \textcolor{blue}{(SELECT Avg(singer.Age) FROM singer} \\
    \textbf{Gold SQL}: SELECT Song\_Name FROM singer WHERE Age > (SELECT avg(Age) FROM singer) \\
    \midrule
    \textbf{Extra}: Find the average age of students who do not have any pet. \\
    \textbf{Cascaded}: SELECT \textcolor{red}{Student.Fname} FROM Student WHERE Student.StuID NOT IN (SELECT Has\_Pet.StuID FROM Has\_Pet)\\
    \textbf{Wav2SQL}: SELECT \textcolor{blue}{Avg(Student.Age)} FROM Student WHERE Student.StuID NOT IN (SELECT Has\_Pet.StuID FROM Has\_Pet) \\
    \textbf{Gold SQL}: SELECT avg(Age) from Student where stuid not in (select stuid from has\_pet) \\
    % \midrule
    % \midrule
    % \textbf{Medium}: What is the money rank of the poker player with the highest earnings?\\
    % \textbf{Cascaded}: SELECT poker\_player.Money\_Rank FROM poker\_player ORDER BY poker\_player.Earnings Desc LIMIT 1 \\
    % \textbf{Wav2SQL}: SELECT \textcolor{red}{Max(poker\_player.Money\_Rank)} FROM pokerhttps://www.overleaf.com/project\_player ORDER BY \\ poker\_player.Earnings Desc LIMIT 1 \\
    \bottomrule
    \end{tabular}
    \vspace{2mm}
    \caption{Three examples compared with cascaded system. We mark the wrong part of the cascaded model in red while the corresponding correct part in Wav2SQL in blue. The input question is represented by SQL query difficulty. Cell values in the SQL queries are replaced with placeholder "terminal".}
    \label{table:case}
\vspace{-3mm}
    \end{table*}
\input{sections/experiment/performance}

\input{sections/experiment/custom}

\input{sections/experiment/ablation}
\input{sections/experiment/case}


    



    





==> sections/experiment/performance.tex <==
\subsection{Model Performance}
  
For in-domain evaluation, we prepare spoken questions with seen accents and speakers according to different SQL components, including SELECT, WHERE, GROUP, ORDER, AND/OR, and KEYWORD following~\cite{yu2018spider}. The results are compiled and presented in Table~\ref{res:1}, and we have the following observations: Wav2SQL surpasses the cascaded system across almost all SQL component matching and exact match accuracy on all SQL queries. Specifically, the SELECT and WHERE component have increased significantly by 5.0\% and 3.1\% respectively, and exact match accuracy has increased by 2.5\%, demonstrating the effectiveness of our direct speech-to-SQL parsing model. It indicates that our direct S2SQL model avoids error compounding across subsystems. Besides, Wav2SQL greatly surpasses DeepSpeechSQL which proves the superiority of Hubert. Compare to the upper bound less variance dataset constructed by a single-speaker single-accent TTS system, we still achieve competitive performance, indicating the efficiency of our proposed techniques for reducing acoustic attributes and promoting generalization. 

\begin{table}[ht]
    \centering
    \small    
    \vspace{1mm}
    \begin{tabular}{l|c|c|c|c}
        \toprule
        Dataset     & Easy & Medium & Hard & Extra \\
        \midrule
        % \multicolumn{7}{l}{\bfseries Cascaded}            \\
        % \midrule
        DeepSpeechSQL & 29.4 & 10.3 & 11.5 & 6.0 \\
        Cascaded    & 51.2 & 28.3 & \bfseries 26.4 & 16.9 \\
        % \midrule
        % \multicolumn{6}{l}{\bfseries Wav2SQL}                   \\
        % \midrule
        Wav2SQL       & \bfseries 54.8 & \bfseries 29.1  &   25.3  &  \bfseries 25.3 \\
        \bottomrule
    \end{tabular}
    \caption{A comparison to the cascaded model and DeepSpeechSQL model in MASpider according to the level of difficulty.}
    \label{res:diff}
\end{table}

To further verify the effectiveness of our methods, we compare our model with the cascaded system and DeepSpeechSQL model. We group the parsing difficulty into easy, medium, hard, and extra according to the number of component selections and conditions of the target SQL queries. As illustrated in Table~\ref{res:diff}, we have the following observations: 

1) As parsing difficulty increases, a distinct degradation could be witnessed in generation accuracy; and 2) our direct speech-to-SQL parsing model outperforms the cascade baseline since it avoids error compounding across subsystems, demonstrating a large margin improvement by 8.4\%, especially in the extra hard part; and 3) Our model is far superior to DeepSpeechSQL at all levels, indicating that the self-supervised Hubert model is more suitable for our task than the traditional ASR Encoder.




==> sections/experiment/setup.tex <==
\subsection{Experimental Setup}
% \vspace{-3mm}

\textbf{Evaluation Metrics} Following the common practice~\cite{yu2018spider}, we evaluate the performance by exact match accuracy and component matching accuracy provided by~\cite{yu2018spider}, where exact match accuracy measures whether the predicted query is equivalent to the gold query as a whole while component matching measures the average exact match between the prediction and ground truth on different SQL components.

\textbf{In-domain and Out-of-domain Test Set} The division of in-domain is based on the Spider, resulting in 8659/1034 train/test sets, where speakers and accents are seen during training. Conversely, in the custom out-of-domain split, neither the speaker nor the accent is visible during training, and the train/test split is 8001/1692. It is worth noting that the databases used in these two divisions are invisible.

\textbf{Training and Inference}
We train our model on a single 32G NVIDIA V100 GPU with a batch size of 10 and a gradient accumulation value of 4 for 30k steps using the Adam optimizer with the default hyperparameters. The learning rate increases from 0 to $7.4 \times 10^{-4}$ with training. We preprocess column names and table names for tokenization and lemmatization using StandfordNLP toolkit~\cite{manning2014stanford}. For the pre-trained models, We adopt Hubert-Base to provide speech representation and GloVe~\cite{pennington2014glove} for the textual schema. In inference, we adopt beam search decoding with beam size 1.

 % We hold fixed the word embeddings during training, except for the 50 most common words in the training set. We build the schema linking borrowed from RAT\cite{wang2019rat}. 

\textbf{Model Configurations} 
% Our cross-modal encoder consists of 8 relation-aware cross-modal attention layers with 256 dimensions. 
In the SQL decoder, we set the rule embedding size as 128 and the node type embedding size as 64. Following ~\cite{huang2022transpeech,lee2021direct}, the ASR model in our work is Wav2vec 2.0 Large(LV-60) + Self Training / 960 hours / Libri-Light + LibriSpeech~\footnote{\url{https://github.com/facebookresearch/fairseq/tree/main/examples/wav2vec}}. A comprehensive table of hyperparameters is available in Appendix~\ref{sec:arch} in the supplementary materials.

\textbf{Baseline models} We compare generated SQL queries of our Wav2SQL with other systems, including:
(1) Cascaded: the cascaded model composed of automatic speech recognition(ASR) and text-to-SQL parsing model, which adopts the wav2vec 2.0~\cite{baevski2020wav2vec} and RATSQL~\cite{wang2019rat}.
(2) S2SQL-TTS: the S2SQL model trained on the dataset synthesized as our upper bound, where S2SQL means the model after removing the speech reprogramming, and adversarial learning in our Wav2SQL. The TTS model we adopt here is FastSpeech 2~\cite{ren2020fastspeech}.
% (3) WhispherSQL: This baseline employs the speech encoder of Whispher-Base~\cite{radford2022robust} to replace Hubert as audio features, where other modules are consistent with the S2SQL model.
(3) DeepSpeechSQL: This baseline employs the speech encoder of DeepSpeech~\cite{amodei2016deep} to replace Hubert as audio features, where other modules are consistent with the S2SQL model.

==> sections/introduction/main.tex <==
\section{Introduction}

Speech-to-SQL parsing (S2SQL) aims to generate the SQL query from a spoken question based on relational databases. This technology is highly beneficial as it breaks down barriers among those who lack proficiency in SQL queries and are unable to perform screen inputs while driving or exercising. Furthermore, S2SQL provides flexible and convenient ways of interaction, which opens up a host of practical applications in fields such as vehicle terminals, smart watches, smart speakers, and the medical industry.  Conventional S2SQL systems~\citep{kumar2013system,song2022speech} are often composed of a cascade of two components: automatic speech recognition (ASR)~\cite{yu2016automatic,schneider2019wav2vec,hsu2021hubert} and text-to-SQL parsing~\cite{bogin2019representing,bogin2019global,chen2020measuring,guo2019towards}. Compared to cascaded systems, work on direct S2ST is very limited, with the potential benefits of 1) working on languages without written form~\cite{campbell2008ethnologue}, where an estimated half of the 7,000 languages in the world actually do not have written forms; 2) avoiding error compounding across sub-systems~\cite{nakamura2006atr,jia2019direct}.


The recent development of direct S2SQL parsing still faces several challenges: 1) despite the benefits of direct approaches, model training is faced with the major issue of data scarcity. Human-labeled speech data is expensive to create, there are very few data resources providing parallel speech, and the data amount is quite limited, 2) increasing demand for SQL parsing from personalized speech challenges models especially in unseen scenarios. When the distributions of custom voice (speaker and accent) differ from training data, the system performance deteriorates due to distribution gaps, and 3) the modality gap between the spoken question and text schema hinders the ability of the question schema, making it difficult to align question speech to the intended tables.

To accelerate S2SQL research, we assemble an open-source, multi-speaker, and multi-accent S2SQL corpus MASpider. To the best of our knowledge, MASpider is the first open-source speech-to-SQL parsing dataset. We have attached part of MASpider to the
supplementary materials, and we will release the entire dataset after the paper publication. To overcome the aforementioned challenges in this paper, we propose Wav2SQL for direct speech-to-SQL parsing, which is generalizable to unseen acoustic conditions (speaker and accent) in custom data. To be more specific, 1) leveraging self-supervised learning (SSL)~\cite{baevski2020wav2vec,hsu2021hubert}, it alleviates the data scarcity issue and benefits S2SQL model training, 2) we introduce speech re-programming and gradient reverse technique to effectively eliminate the style attributes in representation, which promote the model generalization to unseen speakers and accents in custom data.
% , and 3) we propose a cross-modal relation-aware fusion architecture which enhances fine-grained question-schema modeling and narrow the modality gap between the spoken question and textual schema.


% have been extensively studied for tackling the data scarcity issue for S2T. In this work, we show that large-scale self-supervised pre-training with monolingual speech and text data and data augmentation techniques that benefit S2T model training can also be applied to S2UT model training.


% Out-of-domain input is often encountered in real human-computer interaction scenarios, and the speech-to-SQL system will experience significant performance degradation in custom scenarios(e.g.unseen speakers or accents). In order to further improve the generalization of the system to different accents, we propose 1) Speech Re-programming, which improves the speech encoder's ability to model different spoken questions by constructing different sample pairs to achieve information enhancement. 2) Domain Adversarial Training, which is designed to remove speaker information from learned representations and improve domain generalization by gradient reverse layer and domain classifier.

% As for the multimodality challenge, one standard solution for audio-text feature fusion is to concatenate the audio features extracted by CNN with the text features obtained by using language model\cite{kampman2018investigating}. This naive strategy is limited by modeling uni-modal features and thus supports only coarse-grained reasoning. With the huge progress made by transformer in vision, we propose a cross-modal relation-aware transformer to capture fine-grained question-schema reasoning and narrow the modal gap.


Experimental results on the MASpider dataset demonstrate that our Wav2SQL model surpasses the cascaded system in the exact match accuracy and achieves competitive performance with our model trained on the TTS dataset. The main contributions of This work are summarized as follows:
\begin{itemize}
    \item We introduce the first cross-domain speech-to-SQL parsing benchmark dataset MASpider\footnote{Audio samples are available at \url{https://Wav2SQL.github.io/}}. 
    \item Leveraging self-supervised learning, we propose the first direct speech-to-SQL parsing and show that the large-scale pre-training alleviates the data scarcity issue.
    \item Through introducing speech reprogramming and gradient reversal technique, we effectively eliminate the style attributes in speech representation and predict the style-agnostic variation, which significantly improves the model generalization to unseen speakers and accents in custom data.
    \item Experimental results on the MASpider dataset demonstrate that our model outperforms the cascaded systems and achieves state-of-the-art performances.
\end{itemize}

==> sections/limitation/main.tex <==
\section{Limitation and Potential Risks}
As mentioned in the model performance, there is still a certain gap between Wav2SQL and S2SQL-TTS. One of our future directions is to further remove accent and speaker information to improve generation performance. In addition, our experiments find that the schema linking we adopt is still rough compared to text schema linking, which seriously affects the performance of our model. In the future work, we will study how to obtain accurate and fine-grained schema linking.


Wav2SQL lowers the requirements for speech-to-SQL generation, which may cause unemployment for people with related occupations databases developers and SQL programmer. Furthermore, there is the potential for leading to the misuse of database than they expect.

==> sections/method/classifier.tex <==
\subsection{Gradient Reversal Classifier}
\label{4.3}
To eliminate the speaker identity in speech representation, we introduce a gradient reversal layer (GRL) in speaker classifier~\citep{ganin2016domain}, which regards speaker variations as a classification problem and directly maximizes the loss of the domain classifier by reversing its gradients. 
In backpropagation, GRL takes the gradient from the subsequent layer and changes its sign by multiplying with -1 before passing it to the preceding layer:
\begin{equation}
    R(x) = x,  \frac{dR}{dx} = -\textbf{I},  \label{1}
\end{equation}
where I denotes an identity matrix.

It ensures that the feature distributions between different speakers are similar (i.e. as distinguishable as possible), resulting in speaker-agnostic features. Therefore, we can further obtain audio features that preserve semantics regardless of accent and speaker, demonstrating better generalization to custom data in SQL decoding.

% Our objective encourages speaker-agnostic features by reducing discrimination among different speakers, from speech features extracted by Hubert\cite{hsu2021hubert}. Equation(\ref{3}) defines a Speaker Prediction(SP) network to predict speaker ID over N speakers.
% \begin{equation}
%     \begin{split}
%         \rm{MP}(x) &= \frac{\sum_{i}(x_i)}{|x|} \\
%         \rm{SP}(x) &= \sigma(\rm{MP}(LSTM(x)))W_s + b \label{3}
%     \end{split}
% \end{equation}
% where MP is the mean-pooling layer, the activation function is tanh, $ W_s\in\mathbb{R}^{N\times|x|} $ is a weight and $b\in R^N$ is a bias.


% Finally, Equation~\ref{5} defines the classification loss function in order to obtain speaker-invariant representations:
% \begin{equation}
%     \mathcal{L}_{CE} = -\sum_{x}(\log p(s|x))\label{5}
% \end{equation}

% \subsection{Cross-Modality Fusion}
% \label{4.4}
% In direct speech-to-SQL parsing, alleviating the modality discrepancy between table columns and the spoken question could be an open problem. Leveraging recent progress on vision transformer~\cite{arnab2021vivit} and relation-aware self-attention~\cite{wang2019rat}, we attend to column items and table names and find out how schema contributes to the question.


% % As such, we propose to attend to column items and table names to reason how schema contributes to the question, leveraging recent literature on the vision transformer architecture and relation-aware self-attention\cite{arnab2021vivit} in RATSQL\cite{wang2019rat}.

% % One standard solution for audio-textual feature fusion is to represent audio as a matrix representation as it varies with time by self-supervised speech representation model and concatenates with text features from the language model. This fusion strategy is limited by modeling uni-modal features and thus supports only coarse-grained reasoning. However, 

% Specifically, after the self-attention module, we follow the two cross-modality Fusion modules to fine-grained modeling of the two different modalities of question(Q) and schema(S) by using cross attention and injecting pre-defined edges. The formula for cross-modality fusion is presented as follows:
% \begin{equation}
% \label{6}
% \begin{split}
%     e(q_i,s_j) &= \frac{q_i W_Q(s_j W_K+\mathbf{R}_{ij})^T}{\sqrt{d_k /H}}) \\
% z(q_i, s_i) &= softmax(e_{ij})(s_i W_V + \mathbf{R}_{ij})
% \end{split}    
% \end{equation}
% where $\mathbf{R}_{ij}$ is the learned edge feature to represent the predefined cross-relation between the question item and the schema item, H is the number of heads, $W_Q \in \mathcal{R}^{d_{model} \times d_k } $, $W_K \in \mathcal{R}^{d_{model} \times d_k }$, and $W_V \in \mathcal{R}^{d_{model} \times d_v }$ are the linear layer parameter matrices of query, key, and value.
% This relation-aware cross-modal attention allows the spoken question to interact with different items of the schema and align the question utterance to the intended columns or tables. After passing $Q_i$ and $A_j$ through N encoder blocks, we obtain the fused audio-textual feature sequence, which is then sent to the SQL decoder.

==> sections/method/decoder.tex <==
\subsection{SQL Decoder}
\label{4.4}
The SQL decoder follows the grammar-based architecture of ~\cite{yin2017syntactic}, which generates the SQL as an abstract syntax tree(AST) in depth-first traversal order. The generation process of SQL AST is factorized into sequential actions, which are divided into two cases: (1) \textsc{ApplyRule} which expands the last generated node according to the grammar rules or completes a leaf node, (2) \textsc{SelectColumn} and \textsc{SelectTable} represent that selects a column or table item from the schema respectively.


Firstly, the probability of generating a SQL y is defined as:
$$p(y|x) = \prod_t{p(a_t|x,a_{<t})} $$
where $x$ is the encoded memory of questions, columns, and tables, $a_t$ is the action token at time step t, and $a_{<t}$ is the sequential actions before time step t. Then in the tree-structured LSTM decoder, the hidden states at each time step t are updated as $m_t,h_t = \rm{LSTM}([a_{t-1};p_t;c_t;n_t], m_{t-1},h_{t-1})$, where $m_t$ is the cell state of time step t, $h_t$ is the hidden state, $a_{t-1}$ is the previous action embedding, $p_t$ is the parent information of the current node, $c_t$ is the context vector, and $n_t$ is the embedding of the current node type. The parent information contains the hidden state and embedding of parent action. The context vector is computed using multi-head attention upon $x$ and $h_{t-1}$. Finally, how action probabilities $p(a_t|x,a_{<t}$ are computed are explained as follows: \\
\\
For \textsc{ApplyRule} action, 
\begin{equation}
p(a_t=\rm{AR}[r]|x,a_{<t}) = softmax_R(g(h_t))
\end{equation}
where $\rm{AR}$ is the \textsc{ApplyRule} action and $g(\cdot)$ is the feed-forward network that is composed of two linear layers and a $tanh$ activation function.
\\
For \textsc{SelectTable} action,
\begin{equation}
    \gamma_j = softmax_j(\frac{(h_tW_Q)(x_jW_K+\mathbf{R}_{ij})^T)}{\sqrt{d}}),
\end{equation}
\begin{equation}
    p(a_t=\rm{ST}[i]|x,a_{<t}) = \sum_j{\gamma_j}
\end{equation}
where ST denotes \textsc{SelectTable} action. The calculation of \textsc{SelectColumn} action is similar.

==> sections/method/encoder.tex <==
\subsection{Enhanced Speech Encoder}
\subsubsection{Self-Supervised Pre-training}
\label{4.2.1}
To alleviate the data scarcity issue~\citep{huang2023make,huang2023audiogpt} and learn linguistic content from raw waveform~\citep{huang2022transpeech,huang2022prodiff,lam2021bilateral}, we leverage recent progress in large-scale self-supervised learning with Hubert~\cite{hsu2021hubert}, with a multi-layer convolution waveform encoder to generate the feature sequence followed by a Transformer~\cite{vaswani2017attention} context encoder to build the contextualized representations. 

We adopt the Hubert-Base model as speech representation, which is pre-trained on 960 hours LibriSpeech~\cite{panayotov2015librispeech}. Notably, speech representations~\citep{choi2021neural} are found to merge not only rich acoustic information but also acoustic attributes related to accents and speakers. To reduce domain-specific variations for better generalization, we investigate a novel technique in the following parts, which effectively eliminates accent and speaker information in speech representations while preserving linguistic content. 


\subsubsection{Analysis: Audio Representation Quality
 Across Layers}

Before introducing our techniques for removing accent and speaker information, we first discuss the impact of the selection of different layers of Hubert on the model performance. Similar to natural language understanding, exploring the transformer layers of the BERT model shows that the underlying blocks encode syntactic information, while high-level semantic information appears in higher blocks. To make a more intuitive sense of this, we separately extract frozen representations of Hubert's 12 layers as audio features. We then input these audio features into the S2SQL model and evaluate their performance by exact match accuracy. Figure ~\ref{fig:layer} demonstrates that the first 7 layers as well as the final layer have poor performance compared to layers 8 to 11 whose accuracy is higher than 29.0 \%. Layer 9 achieves the best accuracy of 33.1 \%. 

 \begin{figure}[ht]
    % \vspace{-5mm}
    \centering
    % \includegraphics[scale=0.5]{figs/layer.pdf}
    \includegraphics[width=0.5\textwidth]{figs/layer.pdf}
   \caption{Speech-to-SQL generation using representations from different Hubert layers pre-trained on LibriSpeech. EM Acc: Exact match accuracy. } 
    \label{fig:layer}
    \vspace{-4mm}
  \end{figure}
% present speech reprogramming to assist in

\subsubsection{Re-program on Acoustic Condition}
\label{4.2.2}
An intuitive way~\cite{li2018domain,bui2021exploiting} to achieve better generalization is to decompose a model into the domain-agnostic and domain-specific parts via disentangled representation learning and eliminate the domain-specific variations.

In contrast, the representation derived from self-supervised models contains not only rich linguistic content but also information related to pitch and speaker, which are style-specific attributes that may decrease model generalization. As such, we conduct re-programming on speech attributes and perturb the rhythm, pitch, and energy information, which disentangle acoustic variation and selectively extract only the linguistic-related information, exhibiting better generalization to unseen custom data. As shown in Figure~\ref{fig:2}{a}, we apply bottlenecks on acoustic conditions and create re-programmed speech samples. Additional details have been attached in Appendix~\ref{sec:ap}.



\paragraph{Rhythm} Rhythm characterizes how fast the speaker utters each syllable. To perturb rhythm information, we adopt random resampling $RR$ to divide the input into segments of random lengths, and we randomly stretch or squeeze each piece along the time dimension. 

\paragraph{Pitch} Pitch is an indispensable component of intonation. First, We normalize the pitch contour to a common mean and standard deviation, removing the timbre variations in speech. Secondly, a chain function is adopted to randomly shift the pitch contour. 

\paragraph{Energy} Energy represents the magnitude of the raw waveforms and visually reflects the volume of the speech. We re-program energy attributes and create samples with different energy distributions.

==> sections/method/main.tex <==
\section{Proposed Method}
\label{4}
\input{sections/method/overview}
\input{sections/method/encoder}
\input{sections/method/classifier}
\input{sections/method/decoder}
\input{sections/method/training_infer}










==> sections/method/overview.tex <==
\subsection{Overview}
\label{4.1}
The overall architecture has been presented in Figure~\ref{fig:2}{b}. To alleviates the data scarcity issue~\citep{huang2022singgan,huang2022fastdiff}, we leverage the large-scale self-supervised models including Hubert~\cite{hsu2021hubert} for the spoken question and language model for the textual schema to derive discriminative representation, enabling direct speech to SQL parsing. For generalizable speech to SQL parsing, we propose several techniques to promote model robustness for unseen (speaker and accent) custom data: 1) we re-program acoustic attributes and perturb the style information in speech, selectively extracting only the linguistic-related information for domain-agnostic modeling; 2) we include gradient reversal classifier to eliminate speaker information with an auxiliary gradient reversal classifier.

% To eliminate the gap between speech and text modal and provide fine-grained question-schema reasoning, we pass the contextual question and schema into the cross-modality fusion encoder (Section~\ref{4.4}). 
In the end, the tree-structure decoder produces results with an abstract syntax tree (AST) in depth-first traversal order. The training procedures are included in Section~\ref{4.5}, and more information has been attached in Appendix~\ref{sec:arch}.

==> sections/method/training_infer.tex <==
\subsection{Training and Inference}
\label{4.5}
We formulate speech-to-SQL parsing as a sequence-to-tree generation problem. The input is the question (audio) and schema (text), which belong to two different modalities, while the output is the SQL query. We adopt the pre-trained self-supervised speech representation model Hubert~\cite{hsu2021hubert} and language model GloVe~\cite{pennington2014glove} as the backbone of our model.
\paragraph{\textbf{Training.}}
\par The final loss terms in training are composed of the two parts:1) domain classification loss $\mathcal{L}_{CE}$: cross-entropy loss between the predicted speaker ID and the ground-truth; 2) SQL generation loss $\mathcal{L}_{MLE}$: maximum likelihood estimation(MLE) based on the given SQL query to maximize the predicted probability $p(y|x, a_{<t})$ based on a given SQL query. Note that, the domain classification loss $\mathcal{L}_{CE}$ is trained to remove speaker information but preserve semantic information, which is helpful for the final objective $\mathcal{L}_{MLE}$ to generate more accurate SQL query and the loss weight of $\mathcal{L}_{CE}$ is set to be 0.01.


\paragraph{\textbf{Inference.}}
\par After training, for each pair of the spoken question and database schema, we generate the target SQL query according to grammar rules with heuristics decode. We replace the special tokens in the target sequences with the SQL keywords.

==> sections/related/domain_generalization.tex <==
\subsection{Domain Generalization}

Domain generalization aims to learn domain-invariant knowledge which can be generalized to target distribution, which attracts attention from researchers~\cite{zhou2020deep,shi2021gradient,tian2022neuron,huang2022generspeech}. ~\cite{li2018deep} propose a conditional invariant adversarial network to learn class-wise adversarial networks and ~\cite{zhao2020domain} learns domain-invariant features by introducing additional entropy regularization to minimize the KL divergence between the conditional distributions of different source domains. For spoken language understanding, unseen speakers and accents in custom data significantly hurt model performance due to the distribution gaps. In this work, we introduce speech reprogramming and gradient reverse to disentangle semantically irrelevant information, leading to the significant promotion of model generalization to custom scenarios.

==> sections/related/main.tex <==
\section{Related Works}
\input{sections/related/text-to-sql}
\input{sections/related/self-supervised}
\input{sections/related/domain_generalization}






==> sections/related/self-supervised.tex <==
\subsection{Self-Supervised Learning in Speech}

Self-supervised speech representation learning encodes the speech feature into context representations. TERA~\cite{liu2021tera} learns speech representation by reconstructing acoustic frames from their altered counterparts. Vq-wav2vec~\cite{baevski2019vq} learns discrete representations via a context prediction task using contrastive loss. Similarly, wav2vec 2.0~\cite{baevski2020wav2vec} is an end-to-end version of vq-wav2vec, while HuBERT~\cite{hsu2021hubert} predicts masked frames pre-quantized using k-means. In this work, we leverage the recent success of self-supervised learning in speech and show that large-scale pre-training alleviates the data scarcity issue and benefits model training.

==> sections/related/text-to-sql.tex <==
\subsection{Text-to-SQL Parsing}

Semantic parsing of natural language to SQL query recently surged in popularity because of the release of two cross-domain datasets-WikiSQL~\cite{zhong2017seq2sql} and Spider~\cite{yu2018spider}. IRNet~\cite{guo2019towards} encodes the question and schema via bi-LSTM and proposes the string match strategy for schema linking. RATSQL~\cite{wang2019rat} presents a unified framework with a relation-aware transformer(RAT) to encode relational databases and NL questions. SADGA~\cite{cai2021sadga} adopts the graph structure to provide a unified encoding model for both the NL question and databases. In recent years, speech-to-SQL systems usually adopt cascaded automatic speech recognition with text-based SQL parsing. However, the error propagation hurts model performance, not to mention that numerous languages do not have written forms. In this work, we present the first direct speech-to-SQL parsing model without using text, which demonstrates the generalization to different accents and speakers.
